Language Models are Hidden Reasoners: Unlocking Latent Reasoning Capabilities via Self-Rewarding

Large language models (LLMs) have shown impressive capabilities, but still struggle with complex reasoning tasks requiring multiple steps. While prompt-based methods like Chain-of-Thought (CoT) can improve LLM reasoning at inference time, optimizing reasoning capabilities during training remains challenging. We introduce LaTent Reasoning Optimization (LaTRO), a principled framework that formulates reasoning as sampling from a latent distribution and optimizes it via variational approaches. LaTRO enables LLMs to concurrently improve both their reasoning process and ability to evaluate reasoning quality, without requiring external feedback or reward models. We validate LaTRO through experiments on GSM8K and ARC-Challenge datasets using multiple model architectures. On GSM8K, LaTRO improves zero-shot accuracy by an average of 12.5% over base models and 9.6% over supervised fine-tuning across Phi-3.5-mini, Mistral-7B, and Llama-3.1-8B. Our findings suggest that pre-trained LLMs possess latent reasoning capabilities that can be unlocked and enhanced through our proposed optimization approach in a self-improvement manner. The code of LaTRO is available at \url{https://github.com/SalesforceAIResearch/LaTRO}.

==> figures/fig-intro-overview.tex <==
\begin{figure}[htbp]
    % \centering
    \begin{tikzpicture}
        \node (query) at (0,0) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=gray, width=5cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                Query $x$: A robe takes 2 bolts of blue fiber and half that much white fiber. How many bolts in total does it take? Let's think step by step.
            \end{tcolorbox}
        };
        \node[below=1cm of query.south west, anchor=north west] (rationales) {
            \begin{tcolorbox}[colback=white, colframe=gray, width=5cm, arc=1mm, valign=bottom, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                \begin{tikzpicture}
                    \node (rationale1) at (0, 0){
                        \begin{tcolorbox}[colback=green!20, colframe=green!20, width=4.5cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                            Rationale $z_1$: A robe takes 2 bolts of blue fiber. It takes half that much white fiber, so it takes 2/2 = 1 bolt of white fiber. To find the total number of bolts, we add the number of blue bolts and the number of white bolts: 2 + 1 = 3. So, it takes a total of 3 bolts of fiber.
                        \end{tcolorbox}
                    };
                    \node[anchor=west] (rationale2) at ([shift={(0,-0.75cm)}]rationale1.south west) {
                        \begin{tcolorbox}[colback=green!20, colframe=green!20, width=4.5cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                            Rationale $z_2$: To make a robe, it takes 2 bolts of blue fiber. It takes half that much white fiber, so it takes $\frac{\text{1}}{\text{2}}\times$2 = 1 bolt of white fiber. So in total, it takes 2 bolts of blue fiber and 1 bolt of white fiber. 2 + 1 = 3.                   
                        \end{tcolorbox}
                    };
                    \node[anchor=west] (rationale3) at  ([shift={(0,-0.4cm)}]rationale2.south west){
                        \begin{tcolorbox}[colback=red!20, colframe=red!20, width=4.5cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                            Rationale $z_3$: The 2 bolts of blue fiber take 2 bolts of white fiber\texttt{<|eot|>}\texttt{<|eot|>}\texttt{<|eot|>}...
                        \end{tcolorbox}
                    };
                \end{tikzpicture}
                Sampled rationales
            \end{tcolorbox}
        };
        \draw[->,dotted] (query.south)--node[left](sample_arrow){\scriptsize Sample}(rationales.north);
        \node[right=0.2cm of sample_arrow.east, anchor=west] (model_q) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=main, width=2.2cm, height=0.6cm, arc=1mm, valign=center, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                Reasoning model $q_\phi$
            \end{tcolorbox}
        };
        \node (groundtruth) at (4.5, 0){
            \begin{tcolorbox}[colback=blue!5!white, colframe=gray, width=3.5cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering                
                Groundtruth $y$: The answer is 3.
            \end{tcolorbox}
        };
        \node (model_p) at (4.5, -1) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=main, width=2cm, height=0.6cm, arc=1mm, valign=center, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                Reward model $p_\theta$
            \end{tcolorbox}
        };
        \draw[->,dotted] (groundtruth.south) -- (model_p.north);
        \node[below=0.18cm of model_p.south, anchor=north] (rewards) {
            \begin{tcolorbox}[colback=white, colframe=gray, width=3cm, arc=1mm, valign=bottom, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                \begin{tikzpicture}
                \node (reward1) at (0,0) {
                    \begin{tcolorbox}[colback=green!20, colframe=green!20, width=2.2cm, arc=1mm, auto outer arc, valign=center, fontupper=\color{black}, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                        \centering
                        ✅ \tiny Reward 1: -16
                    \end{tcolorbox}
                };
                \node (reward2) at (0,-1) {
                    \begin{tcolorbox}[colback=green!20, colframe=green!20, width=2.2cm, arc=1mm, auto outer arc, valign=center, fontupper=\color{black}, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                        \centering
                        ✅ \tiny Reward 2: -12
                    \end{tcolorbox}
                };
                \node (reward3) at (0,-2) {
                    \begin{tcolorbox}[colback=red!20, colframe=red!20, width=2.2cm, arc=1mm, auto outer arc, valign=center, fontupper=\color{black}, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                        \centering
                        ❌ \tiny Reward 3: -256
                    \end{tcolorbox}
                };
                \end{tikzpicture}
                Rewards $\log p_\theta(y|x\oplus z)$
            \end{tcolorbox}
        };
        \draw[->,dotted] (model_p.south) -- (rewards.north);
        \node (mle_loss) at (8, -4) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=main, width=2.5cm, height=0.75cm, arc=1mm, valign=center, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                MLE loss $\Ls^{MLE}$
            \end{tcolorbox}
        };
        \draw[->,dotted] (rewards.east)--(mle_loss.west);
        \node[above=2.5cm of mle_loss.north west, anchor=west] (rloo) {
            \begin{tcolorbox}[colback=white, colframe=gray, width=2.7cm, arc=1mm, valign=bottom, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                \begin{tikzpicture}
                    \node (advantage1) at (0, 0) {
                        \begin{tcolorbox}[colback=green!20, colframe=green!20, width=2.2cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                        ✅ Advantage 1: 118
                        \end{tcolorbox}
                    };
                    \node[anchor=west] (advantage2) at (0, -1) {
                        \begin{tcolorbox}[colback=green!20, colframe=green!20, width=2.2cm, arc=1mm, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                        ✅ Advantage 2: 124
                        \end{tcolorbox}
                    };
                    \node[anchor=west] (advantage3) at (0, -2)  ([shift={(0,0)}]rationale2.south west){
                        \begin{tcolorbox}[colback=red!20, colframe=red!20, width=2.2cm, arc=1mm, auto outer arc, valign=center, fontupper=\color{black}, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                        ❌ Advantage 3: -242
                        \end{tcolorbox}
                    };
                \end{tikzpicture}
                Leave-one-out advantage
            \end{tcolorbox}
        };
        \draw[->,dotted] (rewards.east)--(rloo.west);
        \node[right=0cm of rloo.east] {$\times$};
        \node[right=0.5cm of rloo.east] (likelihood) {
            \begin{tcolorbox}[colback=white, colframe=gray, width=2.7cm, arc=1mm, valign=bottom, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                Log likelihood of rationales $\log q_\phi(z|x)$
            \end{tcolorbox}
        };
        \node (pg_loss) at (11.55, -4) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=main, width=2.5cm, height=0.75cm, arc=1mm, valign=center, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                PG loss $\Ls^{PG}$
            \end{tcolorbox}
        };
        \draw[->,dotted] (likelihood.south)--(pg_loss.north);
        \node[below=1cm of pg_loss.south, anchor=center] (model_q2) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=main, width=2.2cm, height=0.6cm, arc=1mm, valign=center, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                Reasoning model $q_\phi$
            \end{tcolorbox}
        };
        \draw[->, dotted] (pg_loss.south)--node[left](backprop1){\scriptsize Backprop}(model_q2.north);
        \node[below=1cm of mle_loss.south, anchor=center] (model_p2) {
            \begin{tcolorbox}[colback=blue!5!white, colframe=main, width=2cm, height=0.6cm, arc=1mm, valign=center, auto outer arc, fontupper=\color{black}\tiny, boxsep=0.5mm, left=0.5mm, right=0.5mm, top=0.5mm, bottom=0.5mm]
                \centering
                Reward model $p_\theta$
            \end{tcolorbox}
        };
        \draw[->, dotted] (mle_loss.south)--node[left](backprop2){\scriptsize Backprop}(model_p2.north);
    \end{tikzpicture}
    \caption{Overview of Latent Reasoning Optimization using an example query from GSM8K \citep{DBLP:journals/corr/abs-2110-14168}.}
    \label{fig:enter-label}
\end{figure}

==> misc/experiment-v2.tex <==
\subsection{Setup}
We evaluate the performance of the proposed method across two datasets: a mathematical reasoning dataset (GSM8K, \citet{cobbe2021training}) and a logical reasoning dataset (ARC-Challenge, \citet{DBLP:conf/naacl/TalmorHLB19}). The sizes of the datasets are listed in \Cref{tab:datasets}.

\begin{wraptable}{r}{0.47\textwidth}
    \caption{Size of the Datasets}
    \vspace{-1em}
    \label{tab:datasets}
    \begin{center}        
    \def\arraystretch{1}
    \begin{tabular}{c|cc}
        \toprule
        \bf Name & \bf Training & \bf Evaluation \\
        \hline
        GSM8K & 7473 & 1319 \\
        ARC-Challenge & 1119 & 1172 \\
        \bottomrule
    \end{tabular}
    \vspace{-1em}
    \end{center}
\end{wraptable}

\paragraph{Training.}
For each dataset, we fine-tune three base models: Phi-3.5-mini-instruct~\citep{DBLP:journals/corr/abs-2404-14219}, Mistral-7B-Instruct-v0.3~\citep{DBLP:journals/corr/abs-2310-06825}, and Meta-Llama-3.1-8B-Instruct~\citep{DBLP:journals/corr/abs-2407-21783}, abbreviated as Phi-3.5, Mistral-7B, and Llama-3.1-8B, respectively. We provide two baseline comparisons: the base model and the supervised fine-tuned (SFT) model. For GSM8K, LaTRO fine-tuning excludes golden rationales from the solutions in the training set, while the SFT model is trained using golden rationales. For ARC-Challenge, as suggested in~\citep{zheng2024large}, the model is trained to generate answers to the text of multiple-choice questions rather than selecting labels. Since no golden rationales are available for ARC-Challenge, the SFT model is trained to directly generate answers.

\paragraph{Evaluation.}
For GSM8K, we evaluate all models with CoT prompting, and for ARC-Challenge, we evaluate the SFT baseline with direct answer generation, while the base model and the LaTRO fine-tuned model with CoT prompting. All evaluations are conducted with zero-shot prompts. We report both greedy decoding (GD) results and self-consistency (with temperature $T=1$) results. We choose a self-consistency sample size $k=8$ (maj@8) in \Cref{tab:main_experiment} after observing that more than 8 samples did not bring further performance improvement (see \Cref{fig:ablation}~(b) for details).

\paragraph{Implementation.} LaTRO is implemented on the high level as in \Cref{alg:latro_pseudocode}, with additional engineering techniques as discussed in \cref{sec:sampling_control}. LaTRO is implemented using the widely recognized transformers \citep{wolf-etal-2020-transformers} and TRL \citep{vonwerra2022trl} libraries, with PyTorch \citep{Ansel2024PyTorch2F} as backend. DeepSpeed ZeRO \citep{DBLP:conf/kdd/RasleyRRH20} is used in stage 3, along with Flash Attention 2 \citep{DBLP:conf/nips/DaoFERR22} to enhance training efficiency. The models were trained on a machine 
 equipped with 8xH100 80GB GPUs, using bfloat16 precision. %Hyperparameter selections are detailed as follows.
\paragraph{Hyperparameters.} AdamW optimizer with a learning rate of $5\times 10^{-7}$, no warm-up steps, and a linear decay strategy is used. The Monte Carlo (MC) sample size $K=16$ and the batch size of the data loader $3$ are predetermined, resulting in an effective batch size of $48$. Gradient accumulation steps and training batch size are subsequently adjusted to prevent out-of-memory errors during training.
A temperature of $T=1$ is used for MC sampling, and a penalty factor $\gamma=2$ is applied for incomplete rationales. The KL penalty is set at $\beta=0.05$ for GSM8K and $0.25$ for ARC-Challenge. Except for the results presented in \Cref{sec:ablation}, the maximum generation length is maintained at $L=500$. We train all models up to six epochs for GSM8K, and 12 epochs for ARC-Challenge. The checkpoint with best test accuracy is chosen.

For the SFT baseline experiments, we use a batch size of $32$ and adjust the learning rate to ensure that the evaluation loss decreases and finally converges. All SFT baselines are trained for a maximum of 12 epochs. The checkpoint with the best test accuracy is selected. 

In addition to the main quantitative results, we conduct ablation studies on two factors: 1. The maximum generation length $L$, where we study the effects of tuning $L$ in both training and inference times; 2. The self-consistency samples $k$, where we explore to what extent LaTRO can still benefit from inference-time scaling.

The main quantitative results, qualitative analysis of sample responses, and results of the ablation study are presented in \Cref{sec:results,sec:analysis,,sec:ablation}, respectively. Additional details on our prompt templates and more samples can be found in \Cref{sec:templates,sec:sample}.

\subsection{Results}
\label{sec:results}

In this subsection, we present evaluation results that demonstrate how effectively LaTRO enhances the reasoning abilities of LLMs on downstream datasets. The detailed results are provided in\Cref{tab:main_experiment}.

For the GSM8K dataset, LaTRO fine-tuned models outperform all base models by up to $19.5\%$ (Mistral-7B, $47.8\%\rightarrow 67.3\%$) and show an average improvement of $12.5\%$ across the three models examined with greedy decoding. The greatest improvement margin is observed for Mistral-7B, while the smallest is seen for Llama-3.1-8B, consistent with our initial findings in \Cref{fig:logprob_comparison}, where Mistral-7B exhibited the lowest log probability for directly answering questions and Llama-3.1-8B exhibited the highest. With self-consistency, the improvements are by up to $16.5\%$ (Phi-3.5, $74.0\% \rightarrow 90.5\%$) and the average improvement is $13.1\%$. Furthermore, LaTRO models demonstrate superior performance relative to SFT baselines, with an average improvement of $9.6\%$ for greedy decoding and $13.2\%$ for self-consistency. It is worth noting that for the SFT baseline of Llama-3.1-8B, overfitting on the test set is still observed after tuning the learning rate.

For ARC-Challenge, LaTRO fine-tuned models still outperform the baselines, though with a smaller margin. When using greedy decoding, the improvements over the base models are up to $1.6\%$ with an average increase of $1\%$. We see more increment with self-consistency, where the improvement margins are on average $2.4\%$. Comparing to SFT baslines, we find that all three models are very sensitive when fine-tuning to directly generate the answer of ARC-Challenge questions. They perform even inferior to the unoptimized base models. When using greedy decoding, the improvements of LaTRO fine-tuned models over the SFT baselines are on an average of $5.2\%$, and by up to $6\%$ (Llama-3.1-8B). In the case of self-consistency, LaTRO performs better than the base models by an average of $2.4\%$, and surpasses the SFT models by an average of $8.1\%$.
On the less surprising results compared to GSM8K, we conjecture that for ARC-Challenge, the models are already good at producing the answer either directly or through CoT prompting. Hence, further optimization of the reasoning process did not yield significant improvement.

% \haolincomment{Decide later if to add: This also aligns with the findings in \citet{sprague2024cot}, where the authors claimed that CoT only substantially helps with problems that require mathematical, logical, or algorithmic reasoning.}

% \zuxin{We'd better highlight the analysis in the Table, because people may not read the analysis carefully but just look at the results and wonder why we perform poorly on CommonsenseQA. For example, mark GSM8K and ARC as a category that require extensive reasoning and CommonsenseQA as another type.}

% \haolincomment{csqa may be a too easy task for complex reasoning, cite TO COT OR NOT TO COT?CHAIN-OF-THOUGHT HELPS MAINLY ON MATH AND SYMBOLIC REASONING}
% \haolincomment{Here all evaluations are done with $L=500$}

\begin{table}[t]
    \caption{Zero-shot accuracy (\%) comparison between LaTRO and the baselines on GSM8K and ARC-Challenge datasets. The models are fine-tuned on corresponding training datasets. The base model are marked with ``N/A'' in the training method. GD stands for greedy decoding at inference time and maj@8 stands for self-consistency with 8 samples. The models are evaluated by default using CoT, except that $\dagger$ indicates the direct answer generation is applied during evaluation. }
    \label{tab:main_experiment}
    \begin{center}
    %\renewcommand{\arraystretch}{1.35}
    \def\arraystretch{1.3}
    \begin{tabular}{lllcc}
        \toprule
        \bf Base Model & \bf Training Method & \bf Inference Method & \bf GSM8K  & \bf ARC-Challenge \\ 
        \hline
        \multirow{6}{*}{Phi-3.5} & \multirow{2}{*}{N/A} & GD & 72.9 & 85.1 \\
        & & maj@8 & 74.0 & 86.0 \\
        & \multirow{2}{*}{SFT} & GD & 75.8 & 81.0\textsuperscript{$\dagger$} \\
        & & maj@8 & 77.1 & 80.5\textsuperscript{$\dagger$} \\
        & \multirow{2}{*}{LaTRO} & GD & \bf 87.6 & \bf 86.4 \\
        & & maj@8 & \bf 90.5 & \bf 87.5\\
        \hline
        \multirow{6}{*}{Mistral-7B} & \multirow{2}{*}{N/A} & GD & 47.8 & 74.1 \\
        & & maj@8 & 58.2 & 74.1 \\
        & \multirow{2}{*}{SFT} & GD & 57.2 & 70.0\textsuperscript{$\dagger$} \\
        & & maj@8 & 59.9 & 70.6\textsuperscript{$\dagger$} \\
        & \multirow{2}{*}{LaTRO} & GD& \bf 67.3 & \bf 74.3 \\
        & & maj@8 & \bf 73.8 & \bf 78.9 \\
        \hline
        \multirow{6}{*}{Llama-3.1-8B} & N/A & GD & 76.8 & 81.4\\
        & & maj@8 & 79.7 & 84.4 \\
        &  \multirow{2}{*}{SFT} & GD & 73.2 & 77.0\textsuperscript{$\dagger$} \\
        & & maj@8 & 74.7 & 76.4\textsuperscript{$\dagger$} \\
        & \multirow{2}{*}{LaTRO} & GD& \bf 80.1 & \bf 83.0 \\
        & & maj@8 & \bf 87.0 & \bf 85.3\\
        \bottomrule
    \end{tabular}
    \end{center}
    
\end{table}


\begin{figure}[t]
    \centering
     \begin{tabular}{cc}
     \includegraphics[width=.47\linewidth]{figures/ablation_study_token_length.pdf} &
     \includegraphics[width=.47\linewidth]{figures/self_consistency.pdf} \\
     \small{(a) Zero-shot accuracy with different $L$.} & \small{(b) Zero-shot maj@$k$ accuracy with different $k$.}
     \end{tabular}
    \caption{Ablation study results on GSM8K with base model Phi-3.5. In (a), the $x$-axis represents various maximum token length $L$ of reasoning rationales, $y$-axis is the accuracy, and the plot shows the zero-shot performance v.s. various maximum token lengths for different methods. In (b), the $x$-axis represents the \# of sampled reasoning rationales, the $y$-axis is the accuracy, and the plot shows the zero-shot performance v.s. the  \# of reasoning rationales used in the majority vote.}
    \label{fig:ablation}
\end{figure}



\subsection{Ablation Study}
\label{sec:ablation}

In this subsection, we present our ablation study on the effect of different parameters in LaTRO. For consistency, we fix the base model to Phi-3.5 and the dataset to GSM8K throughout the ablation experiments.

% \subsubsection{How many tokens are enough?}
\paragraph{How many tokens are enough?} \citet{DBLP:conf/iclr/0001LZ024} demonstrated that when the input length is $n$, a transformer model with a hidden size of $O(\log n)$ can solve problems equivalent to Boolean circuits of size $m$, using $m$ CoT steps. However, the empirical determination of sufficient CoT tokens for optimal performance remains underexplored. In this section, we report zero-shot accuracy with generation length $L$ ranging from 200 to 1000 tokens at inference time. Additionally, a Phi-3.5 model is fine-tuned with $L=200$ for comparison. We distinguish two LaTRO fine-tuned models, referred to as LaTRO and $\text{LaTRO}_{200}$. As shown in~\Cref{fig:ablation}(a) accuracy gains plateau when $L\geq 500$, suggesting 500 tokens might suffice for grade school math problems. In contrast, limiting $L$ to 200 reduces accuracy, unless the model is trained accordingly. Interestingly, LaTRO significantly improves performance under this constraint by training the model to generate more concise rationales. This finding implies LaTRO can also train LLMs to condense rationales for limited inference-time compute. A sample from $\text{LaTRO}_{200}$ is provided in \Cref{sec:sample} for qualitative analysis.


% \begin{figure}[t]
%     \centering
%     \begin{minipage}{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/ablation_study_token_length.pdf}
%         \caption{Zero-shot accuracy in GSM8K with different $L$}
%         \label{fig:token_length_vs_acc}
%     \end{minipage}
%     \hfill
%     \begin{minipage}{0.45\textwidth}
%         \includegraphics[width=\textwidth]{figures/self_consistency.pdf}
%         \caption{Zero-shot maj@$k$ accuracy in GSM8K with different $k$}
%         \label{fig:self_consistency}
%     \end{minipage}
% \end{figure}
%\subsubsection{How much inference-time scaling is enough?}

\paragraph{Is inference-time scaling still beneficial?} While LaTRO shifts much of the reasoning computation to training time, it can still benefit from the inference-time scaling. To explore this, We evaluate the models again using self-consistency with the number of samples $k$ ranging from 1 to 32. As shown in~\Cref{fig:ablation} (b), with $k=8$ rationales and majority voting, LaTRO achieves 90\% accuracy on GSM8K. This indicates that LaTRO equipped with self-consistency can further enhance performance, even with LaTRO's focus on training-time optimization.


\begin{figure}[ht]
    \centering
    \begin{bluetextbox}
        \setstretch{1.1}
        \textbf{Question}: Frankie and Binkie went bowling together. Frankie's score was 15 better more than twice as high as Binkie's. If Binkie bowled a score of 90, what was Frankie's score? Let's think step by step.

        \textbf{Response (Base model)}: Let's break this problem down into steps:
        
        1. We know that the difference between Frankie's score (F) and Binkie's score (B) is 15. So we can express Frankie's score as \textcolor{red}{F = B + 15}
        
        2. We also know that Frankie's score is twice as high as Binkie's score. So we can write another equation: F = 2B
        
        3. Now, we have two equations with two unknowns. Let's solve for Frankie's score (F) by setting the two equations equal to each other:
        - 2B = B + 15
        - Multiply both sides by 1 to get rid of the fraction: 2B - B = 15
        - Simplify: B = 15 (since subtracting B from 2B results in 15)
        
        4. Now that we know Binkie's score, we can find Frankie's score using either of the equations we created earlier. Let's use the first one (F = B + 15):
        - F = 15 + 15
        - Frankie's score is 30 more than Binkie's score, which is 15 in this case. So Frankie's score is 15 + 15 = 30 + 15 = 45
        
        The final answer is that Frankie's score was 45.

        \textbf{Reponse (SFT)}: Twice as many as Binkie's 90 score is equal to 2*90= <<2*90=180>>180. Therefore, \textcolor{red}{180-(180-15)=165} was the number Frankie bowled. The answer is 165

        \textbf{Response (LaTRO)}: Here's how to solve the problem:
        1. We know that Binkie's score is 90.
        2. The problem states that Frankie's score was 15 better more than twice as high as Binkie's score. This means that Frankie's score is 15 + (2 * 90) = 15 + 180 = 195.

    \end{bluetextbox}
    % \begin{bluetextbox}
    %     \textbf{Question}: Jeff’s work is 3 miles away.  He walks there and back each day he works.  How many miles does he walk if he has to work 5 times a week? Let's think step by step.
    
    %     \textbf{Response (Base model)}: First, let's find out how many miles Jeff walks each day when he works: 1. He walks 3 miles to his work and 3 miles back, so he walks 6 miles for one day.
    
    %     Next, let's find out how many miles he walks in a week if he works 5 days:
    
    %     1. He walks 6 miles each day, so he walks 6 miles * 5 days = 30 miles in a week.
    
    %     So, Jeff walks 30 miles if he has to work 5 times a week.
    
    
    %     \textbf{Response (SFT)}: Each day of work he walks 2 miles because 3 miles/day + 3 miles/day = <<3+3=6>>6 miles. But he walks 5 days a week, so he walks a total of 30 miles a week because 5 days X 2 miles/day = <<5*2=10>>10 miles. The answer is 10.
    
    
    %     \textbf{Response (LaTRO)}: Here is the solution to the problem:
        
    %     1. Jeff walks 3 miles each way he goes to work, so he walks 3 + 3 = 6 miles each day he works.
        
    %     2. If he works 5 times a week, he will walk 6 * 5 = 30 miles each week.
    
    % \end{bluetextbox}
    \caption{Sample responses of a GSM8K question from Mistral-7B models, the errors are highlighted in red.}
    \label{fig:samples_mistral}
\end{figure}



\subsection{Case study}
\label{sec:analysis}
 We take a closer look at the responses generated by the LaTRO fine-tuned models. 
 We select a question from GSM8K and compare the responses from the base, the SFT model, and the LaTRO finetuned model. 
 We choose the set of responses from the Mistral-7B models that we evaluated. As can be seen in \Cref{fig:samples_mistral}, the base model not only generates a lengthy response, it also makes a logical mistake at the first step, where the correct equation to establish here is ``F = 2B + 15''. The SFT model simplifies the answer and makes the first step correct. However, in the second step it first makes a wrong equation, then makes an arithmetic error when evaluating this equation. Further, LaTRO can give a concise and correct answer. We include more sample responses in \Cref{sec:sample}.


==> misc/intro-misc-sep-30.tex <==
% All related keywords:
% Large Language Model;
% Optimizing reasoning capabilities;
% Self-improvement;
% Reinforcement Learning;
% Reward model-free optimization;\haolincomment{should we term 'alignment' or optimization?};

% uncover and activate the LLM internal reasoning capability;
% self-synthesis high-quality reasoning paths (the lack of existing reasoning dataset); 
% maintain the diversity of reasoning paths (compared to sft); 
% training-time self-consistency;

% \zuxin{Maybe we can use the words "The Hidden Reasoner" to describe the main topic of this paper. Like: 1) Unveiling the Hidden Reasoner: Unlocking Latent Reasoning Capabilities in Large Language Models. 2) Your Language Model is Secretly a Hidden Reasoner: Unlocking Latent Reasoning Capabilities in Large Language Models}

% Story-telling Outline:

% 1. Importance of reasoning capability in LLMs \\
% 2. Brief introduction to LLM reasoning capabilities \\
% 3. Challenges of direct answer generation for complex problems \\
% 4. The concept of reasoning paths and their importance \\
% 5. Potential of inference scaling (e.g., OpenAI's o1 model) \\
% 6. Lack of research on improving reasoning during training \\
% 7. Challenges in training-time reasoning improvement:
%    a. Lack of high-quality reasoning data for complex problems
%    b. Issues with supervised fine-tuning (SFT) approaches
%    c. Difficulties in reward modeling for RLHF approaches \\
% 8. Key questions to address:
%    a. Existence and activation of innate reasoning capabilities in LLMs
%    b. Methods to invoke reasoning without external models or feedback
%    c. Generating high-quality, diverse reasoning paths
%    d. Principled approach to shift inference-time scaling to training time \\
% 9. Surprising findings and potential of the proposed approach

% Draft Introduction:

% Reasoning is a cornerstone of human intelligence, enabling the resolution of complex problems, the formation of sound decisions, and the navigation in the intricacies of the world \needscitation.

As we strive to develop more capable and aligned large language models (LLMs), enhancing their reasoning capabilities has become a critical area of research. 
However, the inherent next-token prediction nature of LLMs presents a challenge for them to directly generate answers of complex problems that require multiple reasoning steps \citep{wang2022self,huang2023large}. For example, LLMs often struggle to directly provide precise answers to math problems or even simple puzzles like ``How many `r's are in the word 'strawberry'?".
This limitation has driven researchers to investigate various prompting approaches that encourage models to generate reasoning trajectories or rationales—sequences of tokens that provide additional context and step-by-step progression toward the final answer, such as Chain-of-Thought (CoT) \citep{DBLP:conf/nips/Wei0SBIXCLZ22}, Tree-of-Though (ToT) \citep{yao2024tree}, and Program-of-Thought (PoT) \citep{DBLP:journals/tmlr/ChenM0C23} prompting methods.


The recent advancements also show inference-time techniques to improve the reasoning capability of LLMs \citep{wu2024empirical,brown2024large}, as evidenced by the OpenAI o1 model\citep{openai_learning_2024}, which have demonstrated strong ability in many reasoning tasks, including math \citep{cobbe2021training,trinh2024solving,luo2024improve}, coding \citep{jimenez2023swe,guo2024deepseek,zhang2024diversity}, and science problems \citep{rein2023gpqa}. 
Among these approaches, CoT with Self-Consistency (CoT-SC) \citep{DBLP:conf/iclr/0002WSLCNCZ23} and CoT-Decoding \citep{wang2024chain} extend the CoT approach at inference time by generating multiple reasoning paths and selecting the most consistent one. Additionally, methods like ReAct \citep{DBLP:conf/iclr/YaoZYDSN023} and Reflexion \citep{DBLP:conf/nips/ShinnCGNY23} integrate reasoning into LLM agent loops, further enhancing problem-solving capabilities.

These approaches demonstrate great promise to elicit the reasoning capabilities in during the inference time \citep{snell2024scaling}. However, how to explicitly improve the reasoning abilities during the training phase of LLMs still remains a challenging problem. Several challenges impede progress in this direction. Firstly, there is a scarcity of high-quality reasoning data for complex problems, making it difficult to apply traditional supervised fine-tuning (SFT) approaches. Furthermore, even when such data is available, SFT on deterministic reasoning paths may lead to a lack of diversity in problem-solving strategies, potentially causing over-confidence issues and performance degradation \cite{cobbe2021training}. This is particularly concerning in domains requiring multiple valid approaches, such as mathematical proofs or ethical reasoning.

Another type of approach, which improving reasoning through reinforcement learning from human feedback (RLHF) presents its own set of challenges. Developing a reward model capable of accurately evaluating the quality and validity of reasoning paths is a formidable task, possibly subject to distribution shifts and biased evaluations.

Given these challenges, our research aims to address several fundamental questions:
\begin{enumerate}
    \item Do pretrained LLMs\haolincomment{We actually conducted experiments on instruction fine-tuned versions} already possess innate reasoning capabilities that have not been fully activated or utilized?
    \item If so, how can we invoke and enhance these reasoning abilities without relying on external models or additional human feedback?
    \item Is it possible to generate high-quality reasoning paths while maintaining diversity in problem-solving approaches? \haolincomment{We may need to show this empirically later on otherwise removing this part.}
    % \item Can we develop a principled method to shift the computational burden from inference-time scaling to the training phase, potentially leading to better trade-offs in model performance and efficiency? 
\end{enumerate}

\yy{consider move this to the main method and add a subsection as motivation. }

Our investigations have yielded promising results:
\begin{enumerate}
    \item We find evidence (\Cref{sec:motivating_example}) suggesting that pre-trained LLMs are not only capable reasoners, but also possess the potential to act as explicit reward models for evaluating reasoning paths. We call utilizing such explicit reward functions induced by LLM themselves \emph{self-rewarding}.
    \item Inspired by this preliminary finding, we propose a novel formulation of the reasoning process in LLMs as sampling from a latent distribution (\Cref{sec:formulation}).
    \item We develop latent reasoning optimization, LaTRO, a principled framework that aims to uncover and activate the internal reasoning capabilities of LLMs without the need for extra reward model training or external feedback (\Cref{sec:latro}).
    \item Our experiments show that empirically, by optimizing the rationales, LaTRO outperforms both the base model and the SFT baselines in GSM8K. In addition, our study also suggests that LaTRO is capable of compressing the reasoning process and further moving the compute burden of the inference time to the training time (\Cref{sec:results,sec:ablation}). \needsreview
\end{enumerate}

\haolincomment{Need a conclude of introduction here.}


%\yy{I feel this paragraph we should start with introducing several prompt based reasoning method (cot, self-consistent cot) and how exactly they are used, and then introduce the drawback of these methods.}

% These approaches of generating reasoning trajectories show great promise, with recent work by the OpenAI o1 model \citep{openai_learning_2024}\haolincomment{Not sure if here we should use a citation or a url in the footnote} demonstrating that inference-time scaling can significantly enhance LLM reasoning capabilities. However, a critical gap in the current research community lies in improving these reasoning abilities during training time, rather than relying solely on inference-time techniques.

% Several challenges impede progress in this direction. First, there is a scarcity of high-quality reasoning data for complex problems, making it difficult to apply traditional supervised fine-tuning (SFT) approaches. Moreover, even if such data were available, SFT on deterministic reasoning paths could lead to a lack of diversity in model problem-solving strategies, thus causing the over-confidence issues of the model and lead to potential performance degradation \citep{cobbe2021training}. This is particularly problematic in domains where there are multiple valid approaches, such as mathematical proofs or ethical reasoning.

% Second, the application of reinforcement learning from human feedback (RLHF) to improve reasoning faces its own set of obstacles. Developing a reward model capable of accurately judging the quality and validity of reasoning paths is a formidable task, potentially subject to issues of distribution shift and biased evaluation.


\yy{I feel the intro is too lengthy, maybe a better structure is 1) introduce reasoning; 2) introduce prompt based method and its drawback 3) training based and the challenge 4) several sentences to introduce our main idea and a summary of the content. and control the overall part less than the first two pages}

\input{figures/figure-intro-overview-v2}

\section{Related work}
\paragraph{Reasoning and Math Problem Solving of LLMs}
Prompt-based reasoning methods prove to be effective in many areas like math problem solving, logical reasoning and various kinds of agentic AI tasks. Chain-of-Thoughts or CoT~\citep{wei2022chain} is the pioneering work that prompts the agent to decompose challenging tasks into smaller, more manageable reasoning steps. Tree-of-Thoughts~\citep{yao2024tree}

\paragraph{Variational Bayesian Methods in LLMs}


\paragraph{Self-Improving of LLMs}
\paragraph{Reward Model Free Fine-tuning}


==> misc/intro-misc.tex <==
As we strive to create more capable and aligned artificial intelligence systems, endowing large language models (LLMs) with robust reasoning capabilities has become a critical area of research. Cutting-edge developments in LLMs have showcased their aptitude for diverse reasoning tasks, from logical deduction\needscitation to mathematical problem-solving\needscitation and even creative ideation.\needscitation Nonetheless, the journey towards consistently reliable and diverse reasoning in these models remains challenging and largely uncharted.

The inherent nature of LLMs as next-token prediction engines presents a significant hurdle when tasked with directly generating answers to complex problems. When confronted with a multistep mathematical question or even a tricky word problem, for instance ``how many r's in the word strawberry?", an LLM often finds it difficult to yield a coherent and precise answer without undertaking intermediate stages. This limitation has motivated researchers to explore alternative approaches, such as prompting models to generate reasoning trajectories or rationales, that is, sequences of tokens that provide additional context and step-by-step progression toward the final answer. Along this line of research, there are many effective approaches: Chain-of-Thought (CoT, \citet{DBLP:conf/nips/Wei0SBIXCLZ22}) guides LLM to think by prompting ``Let's think step by step", and Program-of-Thought (PoT, \citet{DBLP:journals/tmlr/ChenM0C23}) offers an alternative reasoning by prompting LLMs to code. CoT with self-consistency (CoT-SC, \citet{DBLP:conf/iclr/0002WSLCNCZ23}) scales CoT at inference time by generating multiple CoT responses and taking the major votes. ReAct \citep{DBLP:conf/iclr/YaoZYDSN023} and Reflexion \citep{DBLP:conf/nips/ShinnCGNY23} bring the reasoning into the LLM agent loops.
\yy{I feel this paragraph we should start with introducing several prompt based reasoning method (cot, self-consistent cot) and how exactly they are used, and then introduce the drawback of these methods.}

These approaches of generating reasoning trajectories show great promise, with recent work by the OpenAI o1 model \citep{openai_learning_2024}\haolincomment{Not sure if here we should use a citation or a url in the footnote} demonstrating that inference-time scaling can significantly enhance LLM reasoning capabilities. However, a critical gap in the current research community lies in improving these reasoning abilities during training time, rather than relying solely on inference-time techniques.

Several challenges impede progress in this direction. First, there is a scarcity of high-quality reasoning data for complex problems, making it difficult to apply traditional supervised fine-tuning (SFT) approaches. Moreover, even if such data were available, SFT on deterministic reasoning paths could lead to a lack of diversity in model problem-solving strategies, thus causing the over-confidence issues of the model and lead to potential performance degradation \citep{cobbe2021training}. This is particularly problematic in domains where there are multiple valid approaches, such as mathematical proofs or ethical reasoning.

Second, the application of reinforcement learning from human feedback (RLHF) to improve reasoning faces its own set of obstacles. Developing a reward model capable of accurately judging the quality and validity of reasoning paths is a formidable task, potentially subject to issues of distribution shift and biased evaluation.

Given these challenges, our research aims to address several fundamental questions:
\begin{enumerate}
    \item Do pretrained LLMs\haolincomment{We actually conducted experiments on instruction fine-tuned versions} already possess innate reasoning capabilities that have not been fully activated or utilized?
    \item If so, how can we invoke and enhance these reasoning abilities without relying on external models or additional human feedback?
    \item Is it possible to generate high-quality reasoning paths while maintaining diversity in problem-solving approaches? \haolincomment{We may need to show this empirically later on otherwise removing this part.}
    % \item Can we develop a principled method to shift the computational burden from inference-time scaling to the training phase, potentially leading to better trade-offs in model performance and efficiency? 
\end{enumerate}

\yy{consider move this to the main method and add a subsection as motivation. }

Our investigations have yielded promising results:
\begin{enumerate}
    \item We find evidence (\Cref{sec:motivating_example}) suggesting that pre-trained LLMs are not only capable reasoners, but also possess the potential to act as explicit reward models for evaluating reasoning paths. We call utilizing such explicit reward functions induced by LLM themselves \emph{self-rewarding}.
    \item Inspired by this preliminary finding, we propose a novel formulation of the reasoning process in LLMs as sampling from a latent distribution (\Cref{sec:formulation}).
    \item We develop latent reasoning optimization, LaTRO, a principled framework that aims to uncover and activate the internal reasoning capabilities of LLMs without the need for extra reward model training or external feedback (\Cref{sec:latro}).
    \item Our experiments show that empirically, by optimizing the rationales, LaTRO outperforms both the base model and the SFT baselines in GSM8K. In addition, our study also suggests that LaTRO is capable of compressing the reasoning process and further moving the compute burden of the inference time to the training time (\Cref{sec:results,sec:ablation}). \needsreview
\end{enumerate}






-----------------------



As we strive to create more capable and aligned artificial intelligence systems, the development of robust reasoning capabilities in large language models (LLMs) has emerged as a critical area of research. Recent advancements in LLMs have demonstrated their proficiency in diverse reasoning tasks, including logical deduction, mathematical problem-solving, and creative ideation. Despite these advancements, consistently reliable and diverse reasoning in these models remains a challenging and largely unexplored area.

The inherent nature of LLMs, which function as next-token prediction engines, presents a significant challenge when directly generating answers to complex problems. For example, LLMs often struggle to provide coherent and precise answers to multistep questions, such as intricate mathematical problems or even simple puzzles like "How many 'r's are in the word 'strawberry'?" without intermediate stages. This limitation has driven researchers to investigate alternative approaches, particularly those that prompt models to generate reasoning trajectories or rationales—sequences of tokens that provide additional context and step-by-step progression toward the final answer.

Among these approaches, Chain-of-Thought (CoT) prompting \cite{DBLP:conf/nips/Wei0SBIXCLZ22} encourages LLMs to think through problems step-by-step. Program-of-Thought (PoT) \cite{DBLP:journals/tmlr/ChenM0C23} offers an alternative by prompting LLMs to generate code as a form of reasoning. CoT with Self-Consistency (CoT-SC) \cite{DBLP:conf/iclr/0002WSLCNCZ23} scales the CoT approach at inference time by generating multiple reasoning paths and selecting the most consistent one. Additionally, methods like ReAct \cite{DBLP:conf/iclr/YaoZYDSN023} and Reflexion \cite{DBLP:conf/nips/ShinnCGNY23} integrate reasoning into LLM agent loops, further enhancing problem-solving capabilities.

These approaches demonstrate significant promise, as evidenced by the recent work using the OpenAI o1 model, which illustrates that inference-time scaling can markedly enhance LLM reasoning capabilities. However, a critical gap in the current research is the improvement of these reasoning abilities during the training phase, rather than relying solely on inference-time techniques.

Several challenges impede progress in this direction. Firstly, there is a scarcity of high-quality reasoning data for complex problems, making it difficult to apply traditional supervised fine-tuning (SFT) approaches. Furthermore, even when such data is available, SFT on deterministic reasoning paths may lead to a lack of diversity in problem-solving strategies, potentially causing over-confidence issues and performance degradation \cite{cobbe2021training}. This is particularly concerning in domains requiring multiple valid approaches, such as mathematical proofs or ethical reasoning.

Secondly, improving reasoning through reinforcement learning from human feedback (RLHF) presents its own set of challenges. Developing a reward model capable of accurately evaluating the quality and validity of reasoning paths is a formidable task, possibly subject to distribution shifts and biased evaluations.

Given these challenges, our research aims to address several fundamental questions:
1. Do pretrained LLMs possess latent reasoning capabilities that have not been fully activated or utilized?
2. If so, how can these reasoning abilities be invoked and enhanced without relying on external models or additional human feedback?
3. Is it feasible to generate high-quality reasoning paths while maintaining diversity in problem-solving approaches?

Our investigations have yielded promising results. Firstly, we find evidence suggesting that pretrained LLMs are not only capable reasoners but also possess the potential to act as explicit reward models for evaluating reasoning paths. We term this utilization of explicit reward functions induced by LLMs themselves as \emph{self-rewarding}. Inspired by this preliminary finding, we propose a novel formulation of the reasoning process in LLMs as sampling from a latent distribution. We develop Latent Reasoning Optimization (LaTRO), a principled framework aiming to uncover and activate the internal reasoning capabilities of LLMs without the need for additional reward model training or external feedback.

Empirically, our experiments show that by optimizing the rationales, LaTRO outperforms both the base model and SFT baselines on the GSM8K dataset. Moreover, our study suggests that LaTRO can compress the reasoning process, shifting the computational burden from inference time to the training phase, thereby leading to more efficient and effective model performance.

In summary, our research contributes novel insights and methodologies for enhancing the reasoning capabilities of LLMs during training, offering a promising direction for future advancements in AI reasoning and problem-solving.
